On the Power of Convolution Augmented Transformer

The transformer architecture has catalyzed revolutionary advances in language modeling. However, recent architectural recipes, such as state-space models, have bridged the performance gap. Motivated by this, we examine the benefits of Convolution-Augmented Transformer (CAT) for recall, copying, and length generalization tasks. CAT incorporates convolutional filters in the K/Q/V embeddings of an attention layer. Through CAT, we show that the locality of the convolution synergizes with the global view of the attention. Unlike comparable architectures, such as Mamba or transformer, CAT can provably solve the associative recall (AR) and copying tasks using a single layer while also enjoying guaranteed length generalization. We also establish computational tradeoffs between convolution and attention by characterizing how convolution can mitigate the need for full attention by summarizing the context window and creating salient summary tokens to attend. Evaluations on real datasets corroborate our findings and demonstrate that CAT and its variations indeed enhance the language modeling performance.

==> app/sel_copy_proof_July3.tex <==
\subsection{Proof of Theorem \ref{sel copy thm}}\label{sel copy proof}

Below we state a generalization of Theorem \ref{sel copy thm} which distinguishes two scenarios: Short convolution with PE and Long convolutions with no PE.
\begin{theorem}[Selective Copy]\label{sel copy thm} Consider the setting of Def.~\ref{sel copy def}. There is a 1-layer CAT $f$ using exponential-decay query-convolution $\Fb_q$ as follows:
\begin{itemize} 
\item Suppose $\Fb_q$ is infinitely long (namely parameterized as an SSM). Then, using $d=|\Sc|+3$ dimensional token embeddings, $f$ solves unique selective copying.
\item Suppose $\Fb_q\in\R^N$ and input sequences contain at most $N$ signal tokens. Using $d=|\Sc|+4$ and 1-D positional encodings, $f$ solves unique selective copying.
\end{itemize}
\end{theorem}


\begin{proof} Let $T$ be the maximum context length the model encounters. Specifically, $T=L+N+1$ where $L$ is the maximum length of the initial input sequence $X$ that precedes the special token $\bot$ and $N$ is the maximum number of signal tokens in $X$. Recall that the cardinality of the signal vocabulary $\Sc$ is allowed to be larger than $N$. Let $\Z=[\X~\bot~\z_{L+2}~\dots~\z_{t}]$ denote the current input sequence where $[\X~\bot]$ is the initial input that kickstarts decoding. We use query convolution thus the CAT model is given by $f(\Z)=\text{nearest\_token\_embedding}(\Z^\top\sft{\Z\W\z^*_t})$ where $\Z^*=\Fb_q\ast\Z$ is the convolved sequence and $\z^*_t$ is the last token of the convolved query sequence for $L+1\leq t\leq T$. We simply set convolution to be the all-ones filter of size $N$ which precisely aggregates the current token and the $N-1$ most recent tokens. %i.e.~of the form $[1~1~\dots~1~0~\dots~0]$ where the objective is aggregating the embeddings of last $N$ tokens. 

%(i.e.~what is meant by \emph{variation} in the theorem statement)
To proceed, we describe the precise problem setting we employ. Concretely, we assume that one of the following two settings hold:\footnote{We require one of these two conditions to state a clean theorem that make no additional assumptions on noisy token embeddings while employing embedding dimension of $d=|\Sc|+4$ for the orthogonal signal-noise token setting and $d=|\Sc|+3$ for the truncated convolution setting.}
\begin{enumerate}
\item \textbf{Orthogonal signal-noise tokens.} The noise token embeddings are orthogonal to the signal token embeddings. Under the setting of the theorem, we can guarantee this by using $|\Sc|$ embedding dimension for the signal tokens and embedding all noise tokens to the same orthogonal token using $D_{\text{noisy}}=1$ additional dimension. More generally, when noisy token embeddings are arbitrary but orthogonal to $\Sc$, the theorem statement will require $|\Sc|+3+D_{\text{noisy}}$ where $D_{\text{noisy}}$ is the dimension of noisy token subspace. %Alternatively, we consider
\item \textbf{Truncated convolution.} Alternatively, rather than vanilla convolution, we use a truncated convolution starting from the $\bot$ symbol, which is the fixed token that kickstarts decoding. This means that, at time $T$, we convolve the elements from $\bot$ to $\z_{T-N-1}$, which removes the influence of the tokens that come before $\bot$.
\end{enumerate}
%Specifically, under the first setting, the required embedding dimension by the theorem will be $N+3+D_{\text{noisy}}$ since we require orthogonal dimensions for noisy tokens and $D_{\text{noisy}}$ will be at least $1$. 
Before proceeding, we add that, the exact same proof described below also works with standard convolution if (i) we pad the initial sequence $X$ with $N$ $\bot$ symbols (rather than using a single $\bot$) to start decoding or (ii) we assume noise and signal token embeddings have sufficiently small correlations (rather than exactly orthogonal). In other words, while we have opted for a clean theorem statement, the result holds under broader/interchangeable conditions.% however, .%cleanest proposed variation is a mild condition that is interchangeable with other related conditions.

\noindent\textbf{Construction.} For solving Selective Copying, we employ a signal encoding to distinguish between the signal and noise tokens and a positional encoding to distinguish the order of the token positions. Concretely, we construct the embedding $\x_i\in\R^{d}$ of each token as follows
\[ 
\x_i=[\x'_i, s_i, p_i].
\] 
Here $\x'_i\in\R^{|\Sc|+D_{\text{noisy}}+1}$ is a unit length \emph{base embedding} vector. $\x'_i$ belongs to a \emph{base embedding} vocabulary $\Sc'\cup\Nc'$. Here $\Sc'$ is the set of orthonormal base embeddings of signal tokens and $\bot$ token (there are $|\Sc|+1$ of them) and $\Nc'$ is the noise embeddings that lie in an orthogonal $D_{\text{noisy}}$ dimensional subspace in $\R^{|\Sc|+D_{\text{noisy}}+1}$.\footnote{For truncated convolution setting, noise and signal tokens can share the same space, thus, we can set $D_{\text{noisy}}=0$. Otherwise, $D_{\text{noisy}}$ can be set as little as $1$ as discussed earlier.} 
%Recall that, if noise and signal tokens are not necessarily orthogonal, we set $D_{\text{noisy}}=0$ and assume embeddings live on $\R^{N+1}$. 

\noindent$\bullet$ \textbf{Signal indicator.} Here, $s_i\in\{0,1\}$ is an indicator of whether the token is a signal token or not. $s_i=1$ for signal tokens and $s_i=0$ for noise tokens. The $\bot$ token is also treated as signal and has the indicator $1$. 

\noindent$\bullet$ \textbf{Position indicator.} $p_i\in\R$ is the position embedding where we simply set $p_i=i/T$ where $T=L+N+1$ is the maximum context length the model encounters where $N$ is the maximum number of signal tokens and $L$ is the initial input length that precedes the special token $\bot$.

\noindent$\bullet$ \textbf{Signal embeddings.} We set signal embeddings $\Sc\cup \{\bot\}$ to be elements of the standard basis. Noise tokens are arbitrary and unit length, as long as the aforementioned assumptions hold.

\noindent$\bullet$ \textbf{Construction of the attention model.} We construct the attention model with the following criteria in order:
\begin{enumerate}
\item The model should always select signal tokens.
\item The model should select a signal token not previously selected.
\item The model should select the farthest signal token from the current/last token.
\end{enumerate}
To satisfy the three criteria above, we pick the attention weights $\W$ as follows
\begin{align}
\W=\begin{bmatrix} -\alpha\Iden_{N+1+D_{\text{noisy}}} & 0 &0\\0 & \beta &0\\0 &0&-\theta\end{bmatrix}.\label{w att choice}
\end{align}
We let $\alpha,\beta,\theta>0$ to be sufficiently large scalars and similarly choose $\beta/\alpha,\alpha/\theta$ to be sufficiently large (i.e. both the scalars and their relative ratios are chosen to be suitably large). We will solve the problem inductively. Suppose that there are $N'\leq N$ unique signal tokens in $X$ and that until $L+1\leq t\leq L+N'+1$, the model outputs the correct sequence of $t'=t-L-1$ unique signal tokens. We will prove that it will accurately output the next signal token in line. 

First observe that the last two coordinates of $\z^*_t$ are strictly positive numbers that are always lower bounded below. The reason is that $\bot$ is included in the convolution of $\z^*_t$ and the positional encodings are also strictly positive scalars. As a result, suppose $\z^*_t=[\z'^*_t~s~p]$ where $s,p>0$. Given a token $\x_i=[\x'_i~s_i~p_i]$, through \eqref{w att choice}, we have that
\[ 
\text{score}_i=\x_i^\top\W\z_t=-\alpha \li\z'^*_t, \x'_i\ri+\beta s s_i-\theta p p_i.
\] 
%\redp{Revise one last time}
Observe that $\li\z'^*_t, \x'_i\ri, ss_i,pp_i$ are all absolutely bounded terms. Thus, by controlling the relative ratios of the scalar knobs $\beta>\alpha>\theta$, we can enforce the three criteria listed above. Let $j$ be the index of the unique signal token that has not been output yet and that should be output next. We will prove that $j=\arg\max_{1\leq i\leq T}\text{score}_i$. This way, by sufficiently scaling $\alpha,\beta,\theta$ proportionally, $f(\Z)$ will output the token at the $j$'th position by saturating the softmax probability at the $j$'th position. First, observe that $j$ cannot already be in the context window of the convolution filter. The window already contains the $t'$ generated signal tokens and the $\bot$ token at its final $t'+1$ positions. On the other hand, since there are $N'$ unique signal tokens, there are still $N'-t'-1$ signal tokens that are ahead of $j$ (i.e.~that occurs after $j$ within the context window). Thus, $j$ also cannot belong to the initial $N-t'-1$ entries of the length $N$ convolution window. Secondly, observe that $\text{score}_j>\text{score}_i$ for all noise tokens $i$. The reason is that, for noisy tokens $s_i=0$ thus $\beta\cdot s$ multiplier will dominate the score for token $j$. Thirdly, if $i$ is a signal token that belongs to the first $t'$ signal tokens model already output, then $\text{score}_j>\text{score}_i$ because for $j$'th token $\li\z'^*_t, \x'_i\ri=0$ whereas for $i$'th token $\li\z'^*_t, \x'_i\ri\geq 1$ and we assumed $\alpha$ dominates $\theta$. Finally, if $i$ is a signal token that comes after $j$, then $\text{score}_j>\text{score}_i$ because $pp_j<pp_i$. Combining these and letting $\alpha,\beta,\theta$ be sufficiently large, we conclude with the proof.
%We will prove that $j$ is the left-most unique signal token that has not been output yet.
\end{proof}
